Neural relation extraction: a survey

Neural relation extraction discovers semantic relations between entities from unstructured text using deep learning methods. In this study, we present a comprehensive review of methods on neural network based relation extraction. We discuss advantageous and incompetent sides of existing studies and investigate additional research directions and improvement ideas in this field.

==> approach.tex <==
In this section, we categorize neural relation extraction methods regarding their assumptions on expressiveness of training instances about the relations. 

\subsection{Sentence-level relation extraction}
\label{sl-re}
In this approach, sentence-based annotated training data is used. Annotation contains sentence-triple alignment information, such that sentences in the training set are labeled with the triples. 
Once trained, the model's objective is to predict new relations given new entity pairs.
% Distant supervision is not required in sentence-level relation extraction since annotated training data is available and assumed to be sufficient.
However, insufficient amount of training data is a major drawback as labeled data is not always available in real life scenarios. Table \ref{tab:sentence-level-dataset} shows total number of relations and sentences provided in common relation extraction datasets according to OpenNRE framework \citep{han2019opennre}. 

\begin{table}[h!]
\caption{Number of relations and sentences provided in common relation extraction datasets.}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
\textbf{Dataset} & \textbf{\#relations} & \textbf{\#sentences} \\
\hline
SemEval-2010 Task 8 & 9 & 6,647 \\ 
TACRED  & 42 & 21,784 \\ 
Wiki80 & 80 & 56,000 \\ 
\hline
\end{tabular}

\label{tab:sentence-level-dataset}
\end{center}
\end{table}

\subsection{Bag-level relation extraction}
\label{bag-re}
% Bag-level relation extraction methods incorporate distant supervision. 
% As seen in Table~\ref{tab:sentence-level-dataset} and based on the given datasets, average number of sentences (instances) per relation (classes) is about $\#650$ for model training. 
Since labeling data in deep learning requires a lot of manual effort, external knowledge bases are used to enhance weakly labeled training set. Knowledge graphs contain information regarding the relations between the entities in the form of ($head$, $relation$, $tail$) triples. For creating distant supervision datasets such as NYT, entity pairs in a triple are aligned with sentences that contain $head$ and $tail$ entities in the natural text. In this approach, the sentences matched by an entity pair constitute a bag. For this reason these datasets are noisy. Besides that, they are imbalanced, that is, the instances are not evenly distributed across relations.
 
%The assumption is that the at least one instance in a bag expresses the specified relation. 
There are different selection methods to weigh the expressiveness of a bag's instances. One might choose a maximum, average or attention selector which considers the most relevant instance, all instances or weighted average of all instances, respectively \cite{riedel2010modeling, hoffmann2011knowledge, lin2016neural}. More details regarding this approach is given in section \ref{distant-supervision-type}.
% Distant supervision assumes the responsibility to determine which sentence supports which relation and to what degree it expresses the relation of interest. In other words, distant supervision labels sentences with appropriate relations, and generates an error-prone training set consisting of possibly wrong labeled instances, which in turn are used to train RE models.
%Because of the noise and imbalance in distant supervision datasets, bag-level approach is more appropriate and widely used \cite{riedel2010modeling, hoffmann2011knowledge, lin2016neural}.

\subsection{Document-level relation extraction}
\label{document-re}	
Sentence-level approach lacks in grasping entity pair relations across a document \citep{yao2019docred, quirk2017distant}, that is to say, it ignores relations which can be deduced only by understanding several sentences within a document. This can especially be vital for some domains such as drug-side effect relations in pharmaceutical documents \citep{verga2018simultaneously}. The study of \citet{quirk2017distant} is the first to address this problem in distantly supervised setups and proposes a document-level graph representation to extract more relations. DocRED \citep{yao2019docred} provides a benchmark dataset for document-level relation extraction which contains relations that can only be extracted from multiple sentences. As of today, performance of document-level relation extraction methods fall behind the human performance when it comes to cross-sentence reasoning, therefore this approach needs more effort.

==> challenges.tex <==
Challenges in neural relation extraction regarding available data and existing contextual and structural approaches are presented in this section.

\subsection{Overlapping triples}
% \noindent {\bf Overlapping triples.} 
%A relational fact is often called a triple which is composed of an entity pair and semantic relation between these entities. 
An entity ({\it SingleEntityOverlap}) or even an entity pair ({\it EntityPairOverlap}) may imply more than one relation in a sentence. Most studies identify entities before the relation classification which assumes that each entity pair is assigned to a single relation (see section \ref{supervised}). 
%Since research studies on joint extraction of entities and relations also fail to deal with overlapping relational facts. 
\citet{zeng2018extracting} propose an end-to-end model which considers relation extraction to be a triple generation problem and applies a copy mechanism to cope with overlapping triples. Another approach proposed by \citet{takanobu2019hierarchical} admits a hierarchy of high-level relation indicator detection to mine the relations in a sentence and low-level entity mention extraction to match these relation to the corresponding entities. GraphRel, introduced by \citet{fu2019graphrel} is a graph convolutional network based neural model that jointly learns entities and relations. It excels the former methods in solving the overlapping triples problem by incorporating the regional and sequential dependency features of words. Unlike the aforementioned methods, \citet{wei2019novel} offer a new formulation for learning relational triples that first identifies subjects, then the relations with a BERT-based subject tagger module, and finally identifies the objects with a relation-specific object module. 
%The proposed hierarchical tagging framework achieves the state-of-the-art results in terms of extracting multiple relations by overcoming overlapping triples problem.


\subsection{Noise in distant supervision}
% \noindent {\bf Noise in distant supervision.} 
Relation extraction needs large amount of annotated data. 
To handle this problem, recent studies incorporate distant supervision which brings its own drawbacks.
Distant supervision faces the problem of wrong labeled sentences troubling the training due to the excessive amount of noise. Related studies try to remedy this problem by sentence-level attention \cite{lin2016neural}, hierarchical attention \cite{han2018hierarchical}, multi-lingual knowledge extraction \cite{lin2017neural}, joint extraction with knowledge graphs \cite{han2018neural} or introducing human annotation to relation extraction \cite{liu2016effective, ratner2016data, zheng2019diag}. %
Detailed information on these methods is given in section \ref{noise}.


%   \subsubsection{Sentence-level attention} \citet{lin2016neural} remedies the wrong labeling problem in distant supervision by incorporating sentence-level attention over multiple instances. After sentence encoding, each sentence is scored with a query-based function according to how well it captures the relation $r$ given an entity pair. This way, noisy sentences are suppressed, informative ones are emphasized.
    
%     \subsubsection{Hierarchical attention} Recent studies mostly handle relations individually, which is a negligent approach towards inter-relatedness of relations. \citet{han2018hierarchical} utilize semantic correlations among relations to build a selective attention in a hierarchical fashion. This approach significantly improves the performance of long-tail relation extraction.
    
%     \subsubsection{Multi-lingual knowledge extraction} Based on the complementarity and consistency properties of different languages, \citet{lin2017neural} combined mono-lingual and cross-lingual attention to take advantage of both language-specific features and the patterns that bear resemblance across languages. They aggregate sentence encodings with weighted attentions to further use in relation prediction. Sequel to this work, \citet{wang2018adversarial} investigate the effect of incorporating adversarial training in relation extraction. To alleviate possible incompetency in finding consistent patterns across different languages, this work defines a discriminator which can determine the language of each instance.
    
%     \subsubsection{Joint extraction with knowledge graphs} Mutual attention of knowledge graphs and text proposed by \citet{han2018neural} aims to discover and leverage the important correspondences of them for each other. In this work, knowledge-based attention denoises textual relation representation, whereas semantic-based attention weighs the relation tags to be fed to textual representation learning.
    
%     \subsubsection{Introducing human annotation}  Recent research papers \citep{liu2016effective, ratner2016data,  zheng2019diag} confirm that including high quality human annotation brings significant improvement in relation extraction by alleviating the noise due to distant supervision. \citet{zheng2019diag} suggest a reinforcement learning based pattern extraction method to ease pattern-writing work for human experts. The pattern-instance pairs are subject to human annotation to be used in fusing the different labeling methods such as distant supervision and relational patterns.

\subsection{Few-shot instances}
% \noindent {\bf Few-shot instances.} 
Few-shot based modelling is especially challenging for NLP tasks, since text data is noisy and human annotators tend to be mistaken in language-specific tasks \citep{gao2019hybrid}. \citet{han2018fewrel} investigate few-shot learning for relation extraction and provide a dataset for this specific task. \citet{gao2019fewrel} improve the former dataset by addressing domain adaptation issues and ``none-of-the-above'' case which adds extra class to the model. Prototypical networks which assume classification models built on prototypes rather than class labels enable the classifier to identify new classes when only few instances are present for each of those \citep{snell2017prototypical, gao2019hybrid}. %\citet{gao2019hybrid} adapted this approach for relation extraction task  and achieved 
%the state-of-the-art results. However, there is still potential of improvement in few-shot instance learning for relation extraction.

% \subsection{Document-level relation extraction}
% % \noindent {\bf Document-level relation extraction.} 
% Sentence-level approach lacks in grasping entity pair relations across a document \citep{yao2019docred, quirk2017distant}, that is to say, it ignores relations which can be deduced only by understanding several sentences within a document. This can especially be vital for some domains such as drug-side effect relations in pharmaceutical documents \citep{verga2018simultaneously}. The study of \citet{quirk2017distant} is the first to address this problem in distantly supervised setups and proposes a document-level graph representation to extract more relations. DocRED \citep{yao2019docred} provides a benchmark dataset for document-level relation extraction with at least $40.7\%$ relations that can be extracted from multiple-sentences. The state-of-the-art relation extraction methods fall behind the human performance when it comes to cross-sentence reasoning, therefore, it expects more effort.

% \subsection{Complicated event detection}
% Event extraction aims to identify different kind of events from text and the appropriate words that imply those events. It differs from relation extraction mainly in the sense that semantic roles of event elements may vary from sentence to sentence they appear in. The deficiency in the input data is a hurdle in complicated event detection. \citet{wang2019adversarial} propose a large event-centric dataset for this purpose. They also incorporate adversarial training to better separate reliable data for event detection from ambiguous instances. Another task in event detection is event argument extraction which mines and categorizes the semantic roles of event arguments. Unlike recent research, \citet{wang2019hmeae} assume such a dependency between event arguments, that some of them are conceptually related based on their argument roles accounting for the concept hierarchy.

==> conclusion.tex <==
In this survey, we summarized neural relation extraction methods in terms of their approaches and data supervision and datasets for this task. In addition, we explained common challenges and discussed possible remedies to them.

To acquire abundant training instances, the latest studies make use of distant supervision. However, it brings noise to data which greatly affects the training of relation extraction models. In addition, there are no explicit negative samples, since the data itself have wrong annotations due to ill-alignment of the unstructured text and the knowledge graph. For that reason, instead of sentence-level approaches in supervised relation extraction, multi-instance approaches are developed for relation extraction with distant supervision. Also, few-shot learning for relation extraction is a research area that has still room for improvement. Supervised approaches are not to be abandoned. Indeed, incorporating pre-trained language models in supervised relation extraction make significant improvements in comparison to using conventional deep learning methods. Instead of treating entity recognition and relation extraction separately as in pipeline approaches, later studies adopt end-to-end approaches jointly extracting the entities and relations, which tend to better handle problems associated with overlapping triples and long-tail relations. 
%Most of the models do not focus on multiple relations, overlapping triples and long-tail relations. End-to-end relation extraction models tend to handle those problems better in the sense that there is no restriction for the number of triples. 
%We discuss possible remedies to common problems that one encounter in relation extraction task.

==> datasets.tex <==
\subsection{Datasets}
%\textbf{SemEval 2010 Task-8 Dataset} 
SemEval 2010 Task-8 Dataset \citep{hendrickx2009semeval} contains 2717 sentences, which do not overlap with the 8000 training instances from the version that was released on March 5, 2010 and the instances from SemEval 2007 Task-4. The dataset has 9 distinct relation type.
%: cause-effect (CE), Instrument-Agency (IA), Product-Producer (PP), Content-Container (CC), Entity-Origin (EO), Entity-Destination (ED).
        
%\textbf{NYT Dataset (NYT10)}
         NYT Dataset (NYT10) \cite{riedel2010modeling}, was created by aligning relations in Freebase with the sentences in the New York Times Annotated Corpus. Training and test set is generated by splitting the dataset by specific years. 
         %from 2005-2006 as training set and from 2007 as test set.
        %  This dataset is also known as NYT10 since the dataset is announced in 2010.
         Numerous previous work used NYT dataset for relation extraction tasks, however they leverage the dataset as their option. 
         
%\textbf{FewRel}    
    % \noindent {\bfseries  FewRel Dataset}\\
        FewRel \citep{gao2019fewrel} is a supervised dataset created to be used in relation classification methods which utilize few-shot approaches. Large set of sentences were first assigned to relations via distant supervision, next, they were annotated by human experts for denoising. The dataset contains 100 relations, each of which has 700 instances. 
        % The average token number in each sentence is 24.99 and the total token number is 124,577.

%\textbf{Wiki80} 
    % \noindent {\bfseries  Wiki80}\\
         Wiki80 is created based on FewRel dataset for few-shot relation extraction tasks, however it is not recognized as a benchmark. It consists of 56,000 samples of 80 distinct relations. The samples are gathered from Wikidata and Wikipedia.

%\textbf{TACRED}    
    % \noindent {\bfseries TACRED Dataset}\\
        TACRED is the crowd-annotated TAC Relation Extraction Dataset developed by The Stanford NLP Group \citep{zhang2017position}. 
        TACRED contains 106,264 samples and 41 relation types with ``no\_relation'' label to indicate that there is no relation between entities.

%\textbf{ACE-2005 Multilingal Training Corpus}
    % \noindent {\bfseries  ACE 2005 Dataset}
         ACE-2005 Multilingal Training Corpus is created for English, Chinese and Arabic languages \citep{walker2005ace} for the 2005 Automatic Content Extraction (ACE) technology evaluation. The datasets consist of various types of annotated data for entities, relations and events.
    
%\textbf{WebNLG}
    % \noindent {\bf  WebNLG}\\
      WebNLG \citep{gardent-etal-2017-webnlg} is another dataset generated for NLP methods. \citet{zeng2018extracting} adapted this dataset for relation extraction tasks. The processed dataset contains 246 relation types, 5019 training, 703 test and 500 validation instances.

\subsection{Evaluation}

For supervised relation classification tasks the standard precision, recall and F-measure are used for evaluation. Authors usually provide the precision-recall curves for their classification results. For distantly supervised relation extraction models, held-out and/or manual evaluation is conducted. The labels of aligned text with a knowledge base are not gold. For this reason, only the relational facts coming from the knowledge base are considered to be true for the test set in held-out evaluation, newly predicted relations are treated as false. Since this assumption does not express the reality, some work (see Table \ref{table:3}) conduct manual evaluation which requires human effort. In few-shot learning, there are configurations in the form of $m$ way $n$ shot, $m$ representing the number of relations (classes), and $n$ representing labeled instance number per relation, in this case, sentences. The models are tested on different configuration of data and accuracy results of models on test set are stated.


==> discussion.tex <==
Neural relation extraction heavily makes use of the research on both deep learning and the semantic web. 
% For instance, distant supervision aligns triples of knowledge bases, which is a field of the semantic web, with the sentences in the natural text.
% Moreover, pre-trained language models are also utilized besides conventional deep learning methods. 
In this section, we discuss possible research directions regarding relation extraction.
%Integrating the research progress on other fields can also give promising results. 

\subsection{Question generation and question answering}
Neural question generation from text is an emerging research field \citep{zhou2017neural, yuan2017machine, kupiec1996method, du2017learning, wolfe1976automatic}. Question-answering on the knowledge graph is also a well-studied research topic \citep{rajpurkar2016squad}. 
%``Squad'' \citep{rajpurkar2016squad} is a well-known question answering system.
Joint use of these studies on question generation from text and question answering on knowledge bases can help to discover missing relations between entities. Appropriate questions can be generated from each sentence using neural question generation methods. Each question is asked to the knowledge graph using question-answering methods that work on the knowledge base. If the system gets a response, then the response can be added to the natural text. Furthermore, a new triple can be generated based on the question and the response, which is appended to the existing triples in the knowledge base. As a result, the training data provides more insights in deep learning methods, as both the natural text and the knowledge graph is enhanced using question generation and question answering methods. 

\subsection{Possible solutions to improve results of attention mechanism}
In relation extraction, attention mechanism usually works best with sentences ranked according to how well they match a specific relation. 
A similarity metric is involved in matching the relation with the sentence. In this regard, various similarity methods can be explored. 
% In addition, possible use of common methods used in information retrieval such as term frequency-inverse document frequency (tf-idf) \citep{luhn1957statistical, sparck1972statistical}, can be explored. 
Based on the results of the relation extraction, importance weights can be refined, until the algorithm comes up with optimum results. 

Another possible approach for improvement is to run event detection algorithms on each of the sentences, paragraphs or documents, and make use of the events in sentence encoding and attention mechanism. 
Once the sentence's event is determined, event type-specific triples can be given a higher ranking to be aligned with the sentence. 
Event detection from a knowledge graph is also an emerging research area \citep{wang2019adversarial, wang2019hmeae}.

\subsection{Multilingual bi-text mining in machine translation}
One possible research field that can be integrated with distant supervision is machine translation using neural network models.
Machine translation models require a comprehensive training corpus which comprises aligned sentences in different languages. 
Consequently, sentence alignment is significant in machine translation. 

Google's Universal Sentence Encoder (USE) \citep{cer2018universal} embeds sentences into vectors by maintaining the context of the whole sentence, with a pre-trained model available for public use. 
An extension to USE which supports multilingual sentence encoding has also been published \cite{yang2019multilingual}. Facebook also published a similar multilingual sentence encoding study called Laser \cite{artetxe2019massively}. These studies make ``bi-text mining'' possible, which captures similarity scores of sentences even if they are in different languages and matches sentences having close similarity scores. 

% Triples used in distant supervision can also be converted to sentences using natural language generation (NLG). Several studies exist for generating natural text from triples \cite{bouayad2014natural,duma2013generating,sun2006domain,cui-etal-2019-kb,triple_to_text}. Once triples are converted to natural text, the problem comes down to bi-text mining, in which studies like USE and Laser can be utilized. It is also possible to align knowledge bases and natural text in different languages using NLG and a multilingual sentence encoding tool. Since most of the general-purpose knowledge bases have more content in English, being able to align them with sentences in different languages can lead to tremendous improvement in distant supervision.
Triples used in distant supervision can also be converted to sentences using natural language generation (NLG). Several studies exist for generating natural text from triples \cite{bouayad2014natural,duma2013generating,sun2006domain,cui-etal-2019-kb,triple_to_text}. Once triples are converted to natural text, the problem reduces to bi-text mining, where pre-trained models such as 
%Google's Universal Sentence Encoder \cite{yang2019multilingual} and Facebook's Laser \cite{artetxe2019massively} can be utilized. 
USE and Laser can be utilized. 
It is also possible to align knowledge bases and natural text in different languages using NLG and a multilingual sentence encoding tool. Since most of the general-purpose knowledge bases have more content in English, being able to align them with sentences in different languages can lead to tremendous improvement in distant supervision.

\subsection{Paraphrasing}
Another improvement in distant supervision can be achieved by expressing sentences in the natural text with different words.
Several paraphrased version of a sentence could be encoded into a vector space along with the original sentence. 
This can help to capture latent words and can result in a higher similarity score with related triples from knowledge bases.
% While denoising methods like attention mechanism filter the unrelated sentences, paraphrasing may still increase the rate of false positives in sentence alignment. One possible solution for reducing the rate of false positive samples is to extend the model with reinforcement learning or adversarial learning. As stated in section \ref{model-textension}, such methods give promising results in noise filtering. 
One possible drawback of this approach could be that while producing abundant data, it simultaneously increases the number of false positives. 
The remedy could be extending the model with reinforcement learning or adversarial learning. 
As stated in section \ref{model-textension}, such methods give promising results in noise filtering. 

\subsection{Possible solutions for document-level relation extraction}
As stated in section \ref{document-re}, current methods on document-level relation extraction give poor results comparing to human performance. 
Enhancing the knowledge base and natural text can be relevant in this scenario, as it assists in finding hidden relation using neural relation prediction methods on the knowledge graph. Besides, external ontologies can be used to enhance the natural text, as ontologies include vocabularies and rule-sets. Locality-sensitive hashing (LSH) methods \citep{datar2004locality, aydar2019improved} could also be adopted to quickly determine which ontology aligns well with the input sentence, paragraph or document. 

\subsection{Integration with few-shot relation extraction}
Modern methods on neural relation extraction filter out instances that do not have a sufficient amount of training data. 
As stated in section \ref{fewshot-re}, few-shot relation extraction is suitable with small amount of training samples. In real scenarios, eliminating instances might not be desired. 
% Instead of filtering datasets, few-shot learning approaches might give better results, where datasets already have an insufficient number of samples. 
As a result, a joint method of neural relation extraction using distant supervision with a few-shot relation extraction algorithm might be more suitable for real-life scenarios.

==> intro.tex <==
Never-ending information generation and sharing on the Web provides us with abundant data, most of which constitute the unstructured text sources. To better make sense of and draw associations among those data, we, human beings, use relational facts among the subjects (entities) in the text. For a more comprehensive understanding of specific domains such as bioinformatics, finance, social networking etc., we need computers to process those information. 

It is essential to represent the information delivered by the text in machine-readable format. One way to do that is to represent entities and their relations in so called triples, which indicate unambiguous facts about entities. A triple ($h$, $r$, $t$) implies that entity $h$ has relation $r$ with another entity $t$.  Knowledge graphs (KG) such as FreeBase \citep{bollacker2008freebase} and DBpedia \citep{auer2007dbpedia} are examples of such representations. They are directed and labeled graph structured data which aim to express such explicit semantics and relations of entities in triple form.

% Neural relation extraction is a sub-task of natural language processing (NLP) that makes use of data-driven deep learning based models for discovering relations between entity pairs given unstructured text data. 
Relation extraction is a sub-task of natural language processing (NLP) which aims to discover relations $r$ between entity pairs $h$ and $t$ given unstructured text data. Earlier work on relation extraction from text heavily relies on kernel based and feature based methods \citep{pawar2017relation}.However, recent research studies make use of data-driven deep learning methods eliminating conventional NLP approaches for relation extraction. \citet{kumar2017survey} explained how the conventional deep learning methods are integrated into relation extraction. \citet{smirnova2018relation} reviewed relation extraction literature focusing on distant supervision. As the number of research studies on relation extraction increases, the need of a survey on current state-of-the-art of neural relation extraction methods arises.

% Human understanding of natural language is guided by existing knowledge regarding the domain, the world, common sense and linguistics. Therefore, it is driven by both data (given data like natural language) and pre-existing knowledge.
% Knowledge-guided NLP methods mimic human learning behavior, such as a deep learning algorithm is guided by an external knowledge base, and extracted knowledge is in turn fed back to the knowledge base itself. In such methods, linguistics and common sense knowledge are represented with sememes (unit of meaning) and word embeddings, while world and domain knowledge is represented by machine-readable knowledge graphs (KGs). 
%You need to explain word embeddings and knowledge graphs in concepts and definitions section
% Distantly supervised neural relation extraction is regarded as a knowledge-guided NLP method, as entity pairs and corresponding relations, namely triples, in the knowledge graph are accordingly aligned with the natural text to be used in model training. 

This work provides a comprehensive and comparative review on the research field, focusing on the challenges together with improvement ideas. 
%Section \ref{concepts} explains basic concepts in neural relation extraction. 
Section \ref{approach} explains various approaches for relation extraction. In section \ref{type} neural relation extraction methods are classified in terms of data supervision and explained. Section \ref{challenges} describes existing challenges in this field of research.  In section \ref{dataset}, commonly used datasets in model assessment are evaluated. We discuss possible future research directions and improvement ideas in section \ref{ideas} and we conclude our survey in section \ref{conclusion}.

%This survey would be useful for three kinds of readers - i) Newcomers in the eld who want to quickly learn about RE; ii) Researchers who want to know how the various RE techniques evolved over time and what are possible future research directions and iii) Practitioners who just need to know which RE technique works best in various settings

%You need to explain word embeddings and knowledge graphs in concepts and definitions section
%In Knowledge Graphs (KG, or KB) knowledge is represented with triples in the form of ( head(subject entity), relation(relation type), tail(object entity) ). Freebase and dbpedia are well known examples of world knowledge graphs.  


%Many applications in information extraction, natural language understanding, information retrieval require an understanding of the semantic relations between entities. 
 
%Part of speech (pos), Named entity recognition (NER), Co-reference and Basic dependencies are tasks of NLP.

%New discoveries in Neural Information Extraction helps understanding the semantics of natural language, however deep learning models are data-hungary as they require significant amount of training data. (lack of data in regular IE, DS might help)

%Knowledge-Guided NLP mimics the same human behaivour: A deep learning algorithm is guided by an external Knowledge Graph, and extracted knowledge is fed back to the Knowledge Graph. (DL + KG). (This is the same behaivour in IE+DS)

==> related.tex <==
%Another paper list: https://github.com/WindChimeRan/NREPapers2019

% In this section, we describe major advances and related studies on neural relation extraction from text, particularly concentrating on distant supervision.


% Regular relation extraction methods are sentence based assuming all relations are contained in sentences. However, some relations can only be inferred from multiple sentences or from the context. Document-level relation extraction aims to extract relations across sentences. \citet{yao2019docred} created a large-scale document-level relation extraction dataset, DocRed, on which they employed regular sentence-level relation extraction methods. The results of their study show that human performance is by far better than the results generated by the automated relation extraction methods, which proves that there is need for research in document-level relation extraction.

% \textbf{Few-shot relation extraction:}
% \label{fewshot-re}	
% Over-fitting is a potential problem in neural relation extraction methods in cases, where the training set only has a couple instances per relation. Few-shot learning is a technique, where only a small amount of training data are available for classification. Few-shot relation extraction solves the over-fitting problem by clustering the samples and training a distance function to the cluster center. New relations are discovered based on the nearest cluster. 

\subsection{Supervised relation extraction}
\label{supervised}
Supervised neural relation extraction from text uses sentence-level relation extraction approach which requires labeled relation-specific training data. Many of the studies on this task rely on classifying entity pairs according to the particular relations they are assigned to. We list the results of existing methods in Table \ref{table:1}.
 % i.	Relation classification:
% 1.	 (Not: NRE paper classifies these as DS but I don’t see DS in these. They are neural network based RE.) attempt to use deep neural networks in relation classification without handcrafted features. (Socher et al., 2012; Zeng et al., 2014; dos Santos et al., 2015) . 
% 2.	“Semantic compositionality through recursive matrix-vector spaces” (a different word, phrase embedding method using recursive matrix model and RNN). 
\subsubsection{Conventional neural models for relation extraction}
Recent research studies focus on extracting relational features with neural networks instead of manual work \citep{socher2012semantic, zeng2014relation, santos2015classifying}. \citet{socher2012semantic} proposes a recurrent deep neural network model which admits a compositional vector representation of words and phrases on a parse tree. Each expression is represented by both a vector and a matrix, the former encodes semantic information of an expression and the latter encodes how much it influences the meaning of syntactically neighboring expressions.
% 3.	+zeng et al 2014- “Relation Classification via Convolutional Deep Neural Network”: (uses convolutional deep neural network to extract lexical and sentence level features, the features are fed into softmax classifier to predict relationship between tow marked nouns. So this is RE with neural networks again.) 

In relation classification, drawing global features of relations within a sentence is a crucial task. Accordingly, \citet{zeng2014relation} utilize convolutional neural networks which can combine local features to obtain a globally representative one.
% 4.	“Classifying Relations by Ranking with Convolutional Neural Networks”: does relation classification using CNN that performs classification by ranking. So this is still RE.
% Uses sentence-level annotated data, cannot be applied to large scale KBs due to the lack of human annotators. So this may not fit into distant supervision. 
To decrease effects of undesirable artificial classes of relations in prediction, \citet{santos2015classifying} introduces a convolutional deep learning model that admits a pairwise ranking loss function and achieves better results than the former model.
%2. 	Yuhao Zhang, et al. 2017. Positionaware attention and supervised data improve slot filling. They use attention too like NRE to select those informative instances. 

TACRED is introduced by \citet{zhang2017position}, a relation extraction dataset created based on yearly TAC KBP evaluations. Proposed LSTM sequence model coupled with entity position-aware attention mechanism trained on TACRED outperforms the TAC KBP 2015 slot filling system.
% LSTM sequence model with position-aware attention mechanism to extract relations. Also new dataset named TACRED is created targeting towards TAC KBP relations using crowdsourcing to better relation extraction. The idea is better supervised data and suitable model make relation extraction more successful.
%3.Zhang and Wang, 2015: Dongxu Zhang and DongWang. 2015. Relation classification via recurrent neural network
% The paper proposes RNN based models have better performance than CNN based models on relation classification tasks. RNN based models tackle problems about long-distance relations and so it is better to capture relations within long contexts.

In \citet{zhang2015relation}'s work, it is claimed that RNN based relation extraction models excel CNN based models, for the reason that CNNs can only capture the local features, whereas RNNs are capable of learning long-distance dependency between entities.
%4.Xu et al., 2015: Yan Xu, Lili Mou, Ge Li, Yunchuan Chen, Hao Peng, and Zhi Jin. 2015. Classifying relations via long short term memory networks along shortest dependency paths; %check if supervised
% The paper offers SDP-LSTM model to classify relations in text. The methodologies of paper can be separated into 3 part; finding shortest dependency path to obtain most relevant information, integrating information using dependency paths, employing custom dropout strategy to avoid over-fitting.

An LSTM model proposed by \citet{xu2015classifying} takes advantage of the shortest dependency path (SDP) between entities. They claim that the words along SDP are more informative. Dependency trees are directed graphs, therefore, there is the need of differentiating whether the first entity is related to the second entity or the relation implies the reverse direction. For this purpose, the SPD is divided into two sub-path, each is directed from the entity towards the ancestor node.
% %5.	 + Thien Huu Nguyen and Ralph Grishman. 2015. Relation extraction: Perspective from convolutional neural networks.
% The article aims to extract relation by using unbalanced dataset and having numerous window sizes of filters. Reducing relation extraction problem to relation classification  is beneficial since relation extraction is more challenging task than relation classification. The system only takes word embeddings as  input feature.
% 6.	+ Shu Zhang, Dequan Zheng, Xinchen Hu, and Ming Yang. 2015. Bidirectional long short-term memory networks for relation classification.
% Relation classification is hard problem to solve since information can be anywhere in sentence. BLSTM (bidirectional long short-term memory) uses lstm systems natural ability combined with dependency parser and ner system.

Uni-directional LSTM models lack in expressing the complete sequential information of the sentences. \citet{zhang2015bidirectional} use bidirectional LSTM model (BLSTM) to better represent the sentences.
% 7.	+Peng Zhou, Wei Shi, Jun Tian, Zhenyu Qi, Bingchen Li, Hongwei Hao, and Bo Xu.2016. Attention-based bidirectional long short-term memory networks for relation classification.
% Finding important information in sentence is challenging task because of important information can be found at any position. BLSTM models is suitable and have proven success to capture information from sentence. The paper adds attention mechanism to blstm model. System takes raw sentences with positional information as input.

Meaningful information can be located anywhere in the sentence. Instead of using features from lexical sources such as dependency parsers and named entity recognizers, \citet{zhou2016attention} incorporate attention mechanism to BLSTM network to capture more informative parts of the sentence.
% ii.	Pipeline approach:
% Some recent studies proposed pipeline approach which jointly extracts relations and relation specific objects \cite{wei2019novel}.  
%1.	(HBT) (2019, Zhepei Wei, Jianlin Su, Yue Wang, Yuan Tian, Yi Chang) “A Novel Hierarchical Binary Tagging Framework for Joint Extraction of Entities and Relations”. Pipeline: extract entities with NER. Apply entity pair classification. Each class is assigned to a relation. Joint extraction of entities and relation.  

Pipeline approaches which first find the entities than match them with the appropriate relations are prone to error-propagation, namely, errors in the first part can't be alleviated in the relation classification part. Recent models study extraction of entities together with their relations. \citet{wei2019novel} introduces a hierarchical tagging scheme that maximizes the likelihood of input data and the relational triples. Given a sentence, first it finds the subjects, then for each relation $r$, it tags the appropriate objects, which can also be an empty set. This way, multiple triples can be extracted.

\subsubsection{Pre-trained language models for relation extraction}
\label{pre-trained}
Transfer learning is commonly used in deep learning to transfer existing knowledge of a model of a specific task to another similar or related task's model. The former models are called pre-trained models and they save plenty of time and computational power. For NLP tasks there are several widely used pre-trained models such as BERT \citep{devlin2018bert}, Transformer-XL \citep{dai2019transformer} and OpenAI's GPT-2 \citep{radford2019language}. 
% explain transofmrers-pretrained lm relation

%While merits of pre-trained models are plenty and remarkable, there are a small number of studies which utilize them in downstream relation extraction tasks. 
Commonly preferred pre-trained language model in relation extraction studies, BERT, is an unsupervised transformer which is trained to predict the next sentence given a sequence of sentences, and also for masked language model. BERT's model captures the contextual information of a word in a given sentence, along with the semantic relation of a sentence to the neighboring sentences in building the whole text. \citet{wu2019enriching} adjust the pre-trained BERT model to handle both sentence and its entities and they achieved better results on SemEval-2010 task 8 dataset than other conventional deep learning methods. \citet{soares2019matching} aim to build task agnostic, efficient relation representations from natural text using BERT. They achieved better results than previous models on SemEval-2010 task 8 and other models trained on TACRED. \citet{zhao2019improving} achieved the best result on SemEval-2010 task 8. They extract graph topological features on top of BERT embeddings. On the other hand, \citet{wei2019novel}, which also utilizes BERT, achieved best results on the distantly supervised NYT dataset.

\begin{table}[h!]
\caption{States F1 scores of supervised relation classification approaches using Semeval 2010 Task-8 as input dataset.}
\begin{center}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c} 
 \hline
 & & \textbf{SemEval 2010} \\ [0.5ex]
 \hline\hline  \multirow{4}{*}{CNN-based}
%   \rowcolor{lightgray}
 & \citet{zeng2014relation}& 82.7  \\ 
& \citet{nguyen2015relation}&  82.8  \\
% \rowcolor{lightgray}
& \citet{santos2015classifying} & 84.1 \\
& \citet{wang2016relation} & 88.0 \\
 \hline\hline
 \multirow{2}{*}{RNN-based}
 & \citet{zhou2016attention} &84.0 \\
 & \citet{cai2016bidirectional} &86.3 \\
 \hline\hline
 \multirow{4}{*}{BERT-based}
 & \citet{wei2019novel} &87.5 \\
 & \citet{soares2019matching} &89.2  \\
 & \citet{wu2019enriching} &89.25 \\
 & \citet{zhao2019improving} &90.2 \\
 \hline
\end{tabular}
%}
\label{table:1}
\end{center}
\end{table}

\subsection{Relation extraction using distant supervision}
\label{distant-supervision-type}
Distant supervision aligns triples in a related knowledge graph with the sentences in input text, in order to automatically generate training data. 
Distant supervision assumes the responsibility to determine which sentence supports which relation and to what degree it expresses the relation of interest. In other words, distant supervision labels sentences with appropriate relations, and generates an error-prone training set consisting of possibly wrong labeled instances, which in turn is used to train relation extraction models. 

\citet{mintz2009distant} is the first to use this technique. The assumption was that given a triple from the knowledge graph, all sentences that contain the head and tail entities of the triple express the corresponding relation. As a matter of fact, it causes wrong-labeling problem. For instance, consider a triple {\fontfamily{qcr}\selectfont (Bill\_gates, Founder, Microsoft)} from knowledge base and two sentences below: 
\\
{\fontfamily{qcr}\selectfont ``Bill Gates is the co-founder of Microsoft.''} and \\
{\fontfamily{qcr}\selectfont ``The greatest mistake of Bill Gates cost Microsoft \\ 
\$400 billion.''}\\
It is clear that the first sentence expresses {\fontfamily{qcr}\selectfont Founder} relation, as the latter does not. Therefore, the training set including the second sentence is said to be noisy or wrongly labeled. Subsequent studies in distant supervision utilized the same trivial idea of triples in sentence alignment as the original paper. However, they differ in the machine learning models and feature encoders along with their approach to sentence labeling with appropriate relations and solving the wrong labeling problem caused by distant supervision. Reader can find the results of existing distantly supervised methods in Table \ref{table:2}.

\subsubsection{Sentence-triple alignment}

%it can be grouped by how the approach solves the wrong labelling problem:
Four different frameworks exist for labeling sentences with appropriate relations, which are \textit{single-instance single-label (SISL)}, \textit{multi-instance single-label (MISL)}, \textit{single-instance multi-label (SIML)} and \textit{multi-instance multi-label (MIML)} learning. Regarding distant supervision, an instance refers to a sentence in the natural text and a label refers to a relation captured by the knowledge base. 
%Single-instance means a particular relation is represented by only one sentence, while in multi-instance approaches a relation can label more than one sentence. Single-label means a particular sentence can be labelled with only one relation, as in multi-label approaches a sentence can be labelled with more than one relations. In this sense, multi-instance multi-label approaches are more realistic, however the model needs to employ efficient ranking and de-noising strategies.  
Single-instance models assume that a particular relation is derived from only one sentence, while multi-instance approach admits more than one sentence to represent a relation. Multi-instance learning is the bag-level distant supervision approach as explained in section \ref{bag-re}.
In single-label methods a particular sentence is relevant to only one relation, whereas in multi-label approach a sentence can express more than one relation. In this sense, MIML learning framework is more realistic, however, it is necessary to employ efficient ranking and denoising strategies.  

Early methods used conventional NLP methods like dependency parsing and POS tagging for denoising strategies in distant supervision. \citet{riedel2010modeling} assume multi-instance approach which is prone to producing noisy labels for training, in case none of the input sentences expresses the relation. \citet{hoffmann2011knowledge} and  \citet{surdeanu2012multi} proposed (multi-instance, multi-label) learning to cover the overlapping triples problem. However, conventional NLP based methods suffer from propagation of errors generated by NLP tools.

Later studies have relied on deep learning methods to solve the wrong-labeling problem in distant supervision.

\subsubsection{Solving wrong-labeling problem with deep learning methods}
\label{noise}
 % 3.	“Distant supervision for relation extraction via piecewise convolutional neural networks.” ((Zeng et al., 2015)):. Multi-instance and piecewise convolutional neural networks (PCNNs). first Multi-instance learning for DS., . 
 % \\
Distant supervision takes on the annotation burden, however it is obliged to wrong labeling problem. Multi-instance learning \citep{dietterich1997solving} aims to relieve problems caused by ambiguously-labeled training data. To denoise training instances of distant supervision, multi-instance learning has become the remedy in relation extraction studies \cite{riedel2010modeling, hoffmann2011knowledge, surdeanu2012multi, zeng2015distant}. \citet{riedel2010modeling} try to remedy wrong labeling with an undirected graphical model. \citet{hoffmann2011knowledge} focus on multi-instance learning with a probabilistic graphical model. Entity pairs in a corpus do not necessarily imply only one relation. In this direction, \citet{surdeanu2012multi} introduce a graphical model with latent variables, which can jointly model the entities and relations in multi-instance multi-label learning fashion.

First neural network model for multi-instance learning with distant supervision was proposed by \citet{zeng2015distant}. 
The method draws relational features with piece-wise convolutional neural network.
% and assumes that at least one sentence that mentions these two entities will express their relation, and only selects the most likely sentence for each entity pair in training and prediction. It is apparent that the method will lose a large amount of rich information contained in neglected sentences. 
The assumption is that, given a relation type, at least one of the input sentences that contain a specific entity pair, is informative, and it considers only the most expressive sentence in training and prediction. Obviously, this method neglects a large amount of data which might also be informative on that relation.
% a.	Other studies selecting one most valid instances: 
% Zeng et al., 2014: “Daojian Zeng et al. 2014b. Relation classification via convolutional deep neural network”; 
% Xu et al., 2015: Yan Xu, Lili Mou, Ge Li, Yunchuan Chen, Hao Peng, and Zhi Jin. 2015. Classifying relations via long short term memory networks along shortest dependency paths; 
%\cite{zeng2014relation} no denoising concern
% \cite{xu2015classifying} no DS
% Santos et al., 2015: Cicero Nogueira dos Santos, Bing Xiang, and Bowen Zhou. 2015. Classifying relations by ranking with convolutional neural networks
% Zhang and Wang, 2015: Dongxu Zhang and DongWang. 2015. Relation classification via recurrent neural network
% \begin{itemize}
%     \item Verga et al., 2016: Patrick Verga, David Belanger, Emma Strubell, Benjamin Roth, and Andrew McCallum. 2016. Multilingual relation extraction using compositional universal schema
%     \item Verga and McCallum, 2016: Patrick Verga and Andrew McCallum. 2016. Row-less universal schema. 
% \end{itemize}
% Zeng et al. (2015): Daojian Zeng, Kang Liu, Yubo Chen, and Jun Zhao. 2015. Distant supervision for relation extraction via piecewise convolutional n
% 3.	(NRE )“Neural Relation Extraction with Selective Attention over Instances” (Lin Et Al): they build sentence-level attention over multiple instances. They claim that Different from their methods, we propose sentence level attention over multiple instances, which can utilize all informative sentences. 

In \citet{lin2016neural}'s work, each sentence is ranked using the attention mechanism based on how well it represents a specific relation. Therefore, it suppresses the noisy ones rooted from distant supervision.
% 5.	Ji et al. 2017 (Distant supervision for relation extraction
% with sentence-level attention and entity descriptions), brings the useful entity information into the calculation of the attention weights. Brings extra information from knowledge bases. 
To better extract the most appropriate relations, especially in ambiguous cases, \citet{ji2017distant} formulate entity descriptors to include background information which operate on the instances weighted by sentence-level attention.  
% 6.	(HNRE) Xu Han, et al. 2018b. Hierarchical relation extraction with coarse-to-fine grained attention. Considers rich semantic correlations among the entities.

Relations are not individual tags, on the contrary, they are in semantic correlation with each other. To incorporate the rich information covered by relational correlations, \citet{han2018hierarchical} apply a hierarchical attention on each bag of instances.
% Note: (Riedel, Yao, and McCallum 2010; Hoffmann et al.
% 2011; Surdeanu et al. 2012; Zeng et al. 2015; Lin et al. 2016;
% Ji et al. 2017) are all bag levels so multi-instance. HNRE is also most probably bag level.
% 5.	Note: studies that incorporates knowledge information: 
% Ji et al., 2017 (Distant supervision for relation extraction with sentence-level attention and entity descriptions); 
% Han et al.,2018: Xu Han, Zhiyuan Liu, and Maosong Sun. 2018. Neural knowledge acquisition via mutual attention between knowledge graph and text)

Another approach is accounting for the information covered by knowledge graphs. \citet{han2018neural} introduce a joint representation learning model for knowledge graph and text, the mutual guidance of which is fed back to the model under an attention mechanism to highlight the significant features of both. % Label-Free Distant Supervision for Relation Extraction
% via Knowledge Graph Embedding
To benefit more from the knowledge graphs, \citet{wang2018label} propose a novel distant supervision approach which refuse the hard labels imposed by regular distant supervision methods, rather, they train the relation classifier directly from KGs with soft labels.
 
Recent research papers \citep{liu2016effective, ratner2016data,  zheng2019diag} confirm that including high quality human annotation brings significant improvement in relation extraction by alleviating the noise. \citet{zheng2019diag} suggest a reinforcement learning based pattern extraction method to ease pattern-writing work for human experts. The pattern-instance pairs are subject to human annotation to be used in fusing the different labeling methods such as distant supervision and relational patterns.

Based on the complementarity and consistency properties of different languages, \citet{lin2017neural} combined mono-lingual and cross-lingual attention to take advantage of both language-specific features and the patterns that bear resemblance across languages. They aggregate sentence encodings with weighted attentions to further use in relation prediction. Sequel to this work, \citet{wang2018adversarial} investigate the effect of incorporating adversarial training in relation extraction. To alleviate possible incompetency in finding consistent patterns across different languages, this work defines a discriminator which can determine the language of each instance.

\begin{table}[h!]
\caption{States mean precision scores of distantly supervised relation classification methods on NYT dataset. ``Held-out'' and`` Manual'' indicates that the scores are from held-out and manual evaluation, respectively.}
\begin{center}
\begin{tabular}{c|c|c} 
 \hline
& & \textbf{NYT}\\ [0.5ex] 
 \hline\hline
 \multirow{4}{*}{Held-out}
& \citet{jiang2016relation} & 72.0  \\
& \citet{lin2016neural} &72.2 \\
& \citet{han2018neural} &71.0 \\
& \citet{han2018hierarchical} &81.6 \\
\hline\hline
\multirow{3}{*}{Manual}
& \citet{zeng2015distant} &78.3 \\
& \citet{ji2017distant} &81.3 \\
&  \citet{wang2018label} &86.9 \\

 \hline
\end{tabular}
\label{table:2}
\end{center}
\end{table}

\subsubsection {Model extensions}
\label{model-textension}
Research studies on relation extraction with distant supervision are not limited to pure deep learning methods. Recent approaches extended their models by incorporating various NLP tools and machine learning methods.
% •	Noise filtering with Adversarial training: \\
%     o	Yi Wu, et al. 2017. Adversarial training for relation extraction.\\

Adversarial learning is used for training classifiers that are robust to both unmodified and perturbed samples. Essentially, it is widely used in supervised learning. \citet{wu2017adversarial} experiment the effects of using adversarial training in relation extraction with distant supervision on convolutional and recurrent neural network architectures and show that it can improve the performance of both.
    % o	DSGAN: Generative Adversarial Training for Distant Supervision Relation Extraction. They recognize the true positive samples from distant supervision dataset before relation extraction. (noise filtering before RE)\\
Redistribution of distantly supervised data can boost the performance of relation classifiers. 
\citet{qin2018dsgan} propose a denoising method for distant supervision relation extraction datasets, in cases where the true positives are more prevalent than the false positives. Similar to generative adversarial networks, this method re-labels the positively labeled instances provided by distant supervision. 
% •	Noise filtering using Reinforcement learning:\\
%     o	Jun Feng et al. 2018. Reinforcement learning  for relation classification from noisy data.\\
Another approach is accounting for reinforcement learning to handle the noisy instances. \citet{feng2018reinforcement} decompose the relation extraction problem into two tasks: instance selection and relation classification. Instance selector is a reinforcement learning agent which selects the most appropriate instance using the relation classifier's weak supervision. 
    % o	Robust Distant Supervision Relation Extraction via Deep Reinforcement Learning. “the goal is to learn to choose whether to remove or remain the distantly supervised candidate instance based on the performance change of the relation classifier”\\
To redistribute the distantly supervised data, \citet{qin2018robust} incorporate reinforcement learning, the policy of which is based on the mere classification performance.

% •	Others:\\
% o	Noise filtering using features extracted from NLP tools:\\
%     	Takamatsu et al 2012. “Reducing Wrong Labels in Distant Supervision for Relation Extraction” build a noise-filtering strategy based on the linguistic features extracted from many NLP tools, including NER and dependency tree, which inevitably suffers the error propagation problem.\\
Other than the aforementioned methods utilizing adversarial networks and reinforcement learning, there are also other advanced training methods to overcome the drawbacks of distant supervision. For instance, \citet{takamatsu2012reducing} utilize a generative model to predict the wrongly labeled patterns in distant supervision. 
% o	Advanced training methods :\\
%     	Tianyu Liu, Kexiang Wang, Baobao Chang, and Zhifang Sui. 2017. A soft-label method for noise tolerant distantly supervised relation extraction . This could be noise filtering too.\\

Unlike studies regarding sentence-level denoising, \citet{liu2017soft} adopt entity pair-level denoising approach and derive soft labels for each entity pair bag, which are subject to change during training.
    % 	Yi Yao Huang and William Yang Wang. 2017. Deep residual learning for weakly-supervised relation extraction\\
Different from the above studies, the noise-tolerant model introduced by \citet{huang2017deep} utilize deep residual learning \cite{he2016deep}.
% o   (Zeng et al., 2017 (Incorporating relation paths in neural relation extraction); 
\citet{zeng2017incorporating} incorporate path relations from text corpus, namely, they build a model which can handle relations that can be driven from several sentences.

\subsection{Relation extraction using few-shot approach}
\label{fewshot-re}
Few-shot learning is a learning method, in which in contrast to regular deep learning methods the amount of available training data is small. The assumption is that reliable algorithms can be built to achieve competitive performance to the models trained with abundant data. We list some studies related to few-shot learning for relation extraction in Table \ref{table:3}.
% Briefly just briefly mention these. One sentence each. This is not our main topic.\\\\
%     i.	Xu Han, et al. 2018c. Fewrel: A largescale supervised few-shot relation classification dataset with state-of-the-art evaluation\\
For the purpose of experimenting few-shot learning algorithms for relation extraction, \citet{han2018fewrel} provide the ``FewRel'' dataset.
    % ii.	Snell et al. 2017,  Prototypical Networks for Few-shot Learning\\
    % iii.	Tianyu Gao et al. 2019. Hybrid attention-based prototypical networks for noisy few-shot relation classification\\
Prototypical networks \cite{snell2017prototypical}, which admit prototypes rather than classes, are used in few-shot learning scenarios for relation extraction\cite{gao2019hybrid}.
    % v.	Livio Baldini Soares et al. 2019. Matching the blanks: Distributional similarity for relation learning.\\
The model proposed by \citet{soares2019matching} outperforms human accuracy on few-shot relation matching.
    % iv.	Zhi-Xiu Ye and Zhen-Hua Ling. 2019. Multi-level matching and aggregation network for few-shot relation classification\\ 
\citet{ye2019multi} introduce an aggregation network model and a matching mechanism which is multi-level.
    % vi.	Zhengyan Zhang, et al. 2019. Ernie: Enhanced language representation with informative entities.\\ %ozgebozal: not few-shot

\begin{table}[h!]
\caption{Accuracy scores of few-shot relation classification methods with the best performing configuration on FewRel dataset.}
\begin{center}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c} 
 \hline
& \textbf{Best configuration} & \textbf{FewRel} \\ [0.5ex] 
 \hline\hline
  \citet{soares2019matching} & 5 Way 1 Shot &88.9 \\
 \citet{gao2019hybrid} & 5 Way 10 Shot &92.06\\
 \citet{ye2019multi} & 5 Way 5 Shot &92.66 \\
 
 \hline
\end{tabular}
%}

\label{table:3}
\end{center}
\end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{c| cc} 
%  \hline
% & Encoder & Dataset\\ [0.5ex] 
%  \hline\hline
%  \rowcolor{lightgray}
% \cite{zeng2014relation}& 82.7 &-  \\ 
% \cite{nguyen2015relation}&  82.8 &-  \\
%  \rowcolor{lightgray}
% \cite{santos2015classifying} & 84.1 &-  \\
% \cite{jiang2016relation} & ????  \\
%  \rowcolor{lightgray}
%  \cite{wang2016relation} & 88.0 &- \\ [1ex] 
%  \hline
% \end{tabular}
% \caption{Stated results of CNN-based methods}
% \label{table:1}
% \end{table}

% Group distantly supervised studies by the embedding and encoders:\\\\
% 1.	CNN based\\
%     a.	CNN based on “Daojian Zeng et al. 2014b. Relation classification via convolutional deep neural network”:\\
%     The CNN model discovers numerous level of feature extraction for given input sentence and it has three components: Word Representation, Feature Extraction and Output. The network needs inputs which include two marked entities and discovers numerous levels of feature extraction of inputs.\\
  
    
    % b.	Settings from Nguyen and Grishman 2015 can be an example\\
    % CNN model can split into 4 part; encoding words, convolution layer which acknowledge n-grams, pooling layer which finds most adequate feature and logistic regression layer with softmax normalization function. \\
    
    
    % c.	Cicero Nogueira dos Santos, Bing Xiang, and Bowen Zhou. 2015. Classifying relations by ranking with convolutional neural networks.\\
    % In this paper authors proposes a novel convolutional neural network which named is Classification by Ranking CNN (CR-CNN) to deal with classification task. This network learns distributed vector representation, which is produced by convolutional layer, of the input text. The idea is calculating a score between vector representation and class representation.\\
    
    
    % d.	CNN with sentence wise pooling. Xiaotian Jiang, Quan Wang, Peng Li, and Bin Wang. 2016. Relation extraction  with multi-instance multilabel convolutional neural networks\\
    % In this paper, CNN architecture is used to extract sentence level feature to build sentence representation. For pooling layer, piecewise max-pooling and cross-sentence max-pooling are used\\
    
    
    
    % e.	CNN with multi-level attention: Linlin Wang, Zhu Cao, Gerard de Melo, and Zhiyuan Liu. 2016. Relation classification via multi-level attention cnns.\\
    % In this paper, a cnn architecture with new objective function, which is better than other loss function, and new form of attention mechanism is employed. The offer.ed attention mechanism has two levels in order to better recognition of patterns in diverse context\\
    
    
    % f.	Lin et al. (2016). NRE paper. Instance level selective attention mechanism.\\\\
    
    
% 2.	PCNN based\\
%     a.	Daojian Zeng, Kang Liu, Yubo Chen, and Jun Zhao. 2015. Distant supervision for relation extraction via piecewise convolutional neural networks\\
    
    
% 3.	RNN based:\\
%     a.	Rui Cai, Xiaodong Zhang, and Houfeng Wang. 2016. Bidirectional recurrent  convolutional neural network for relation classification\\
    
    
%     b.	Peng Zhou, Wei Shi, Jun Tian, Zhenyu Qi, Bingchen Li, Hongwei Hao, and Bo Xu. 2016. Attention based bidirectional long short-term memory networks for relation classification.\\
    
    
% 4.	Bert based: Jacob Devlin, et al. 2019. BERT: pre-training of deep bidirectional transformers for language understanding\\
%     a.	Settings from Soares et al 2019 can be an example.\\
    
    
%     b. HBT paper\\                                


